Interpolating between Images with Diffusion Models

One little-explored frontier of image generation and editing is the task of interpolating between two input images, a feature missing from all currently deployed image generation pipelines. We argue that such a feature can expand the creative applications of such models, and propose a method for zero-shot interpolation using latent diffusion models. We apply interpolation in the latent space at a sequence of decreasing noise levels, then perform denoising conditioned on interpolated text embeddings derived from textual inversion and (optionally) subject poses. For greater consistency, or to specify additional criteria, we can generate several candidates and use CLIP to select the highest quality image. We obtain convincing interpolations across diverse subject poses, image styles, and image content, and show that standard quantitative metrics such as FID are insufficient to measure the quality of an interpolation. Code and data are available at https://clintonjwang.github.io/interpolation.

==> figs/1_teaser.tex <==
% \begin{figure*}[th]
% \centering
% \includegraphics[width=\linewidth]{figs/1_teaser.png}
% \vspace{-12pt}
% \caption{\textbf{Interpolations of real images.}
% By conditioning a pre-trained latent diffusion model on various attributes, we can interpolate pairs of images with diverse styles, layouts, and subjects.}
% \label{fig:teaser}
% \end{figure*}

% \begin{strip}\centering
% \includegraphics[width=\textwidth]{figs/1_teaser.png}
% \captionof{figure}{\textbf{Interpolations of real images.}
% By conditioning a pre-trained latent diffusion model on various attributes, we can interpolate pairs of images with diverse styles, layouts, and subjects.}
% \label{fig:teaser}
% \end{strip}


% \begin{teaserfigure}
% \includegraphics[width=\textwidth]{figs/1_teaser.png}
% \vspace{-8pt}
% \caption{\textbf{Interpolations of real images.}
% By conditioning a pre-trained latent diffusion model on various attributes, we can interpolate pairs of images with diverse styles, layouts, and subjects.}
% \label{fig:teaser}
% \end{teaserfigure}


\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\begin{center}
\centering
\captionsetup{type=figure}
\includegraphics[width=\linewidth]{figs/1_teaser.png}
\vspace{-8pt}
\captionof{figure}{\textbf{Interpolations of real images.}
By conditioning a pre-trained latent diffusion model on various attributes, we can interpolate pairs of images with diverse styles, layouts, and subjects.}
\end{center}}]

==> figs/a_did_scheme.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{figs/a_interp.png}
\caption{``Denoise-interpolate-denoise'' scheme illustrated for generating 3 interpolated frames.}
\label{fig:interp}
\end{figure*}

==> tables/method.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Real image interpolation has unique challenges compared to other tasks that take two images as input.}\label{tbl:performance}
\begin{tabular}{lcccc}
\hline
 & \textbf{Ours} & \textbf{Latent Interpolation} & \textbf{Video Interpolation} & \textbf{Style Transfer}\\
\hline
Image inversion & \checkmark & & \\
Conditioning information & \checkmark & \checkmark & & \\
Pre-trained & \checkmark & \checkmark & & \\
Images of different styles & \checkmark & \checkmark & & \checkmark \\
\hline
\end{tabular}
\end{table}
